A Survey on Knowledge Organization Systems of Research Fields: Resources and Challenges

Knowledge Organization Systems (KOSs), such as term lists, thesauri, taxonomies, and ontologies, play a fundamental role in categorising, managing, and retrieving information. In the academic domain, KOSs are often adopted for representing research areas and their relationships, primarily aiming to classify research articles, academic courses, patents, books, scientific venues, domain experts, grants, software, experiment materials, and several other relevant products and agents. These structured representations of research areas, widely embraced by many academic fields, have proven effective in empowering AI-based systems to i) enhance retrievability of relevant documents, ii) enable advanced analytic solutions to quantify the impact of academic research, and iii) analyse and forecast research dynamics. This paper aims to present a comprehensive survey of the current KOS for academic disciplines. We analysed and compared 45 KOSs according to five main dimensions: scope, structure, curation, usage, and links to other KOSs. Our results reveal a very heterogeneous scenario in terms of scope, scale, quality, and usage, highlighting the need for more integrated solutions for representing research knowledge across academic fields. We conclude by discussing the main challenges and the most promising future directions.

==> main_table.tex <==
\pagestyle{empty}
\newgeometry{margin=1cm}
\begin{landscape}
\section{Classification Schemes and their features}\label{appendixa}

In this appendix, we show a table describing all single-field and multiple-field classification schemes according to the whole set of features available in Sec.~\ref{features}.
For the sake of space, we have reduced the size of some columns (Type of scheme, Kind of hierarchy, Related Terms, Generation) and shortened their values to a single character. Here follows the association between the single letters and their meaning.
\begin{itemize}
    \item \textbf{Type of scheme}: C (\textit{Controlled Vocabulary}), T (\textit{Taxonomy}), U (\textit{Thesaurus}), O (\textit{Ontology})
    \item \textbf{Kind of hierarchy}: M (\textit{mono}), P (\textit{poly})
    \item \textbf{Related Terms}: Y (\textit{yes}), N (\textit{no})
    \item \textbf{Generation}: M (\textit{Manual}), A (\textit{Automatic}), S (\textit{Semi-automatic}), C (\textit{Community-effort})
\end{itemize}



\input{tables/appendix-full-table}
\end{landscape}
\restoregeometry
